FisherSFT: Data-Efficient Supervised Fine-Tuning of Language Models Using Information Gain

Supervised fine-tuning (SFT) is a standard approach to adapting large language models (LLMs) to new domains. In this work, we improve the statistical efficiency of SFT by selecting an informative subset of training examples. Specifically, for a fixed budget of training examples, which determines the computational cost of fine-tuning, we determine the most informative ones. The key idea in our method is to select examples that maximize information gain, measured by the Hessian of the log-likelihood of the LLM. We approximate it efficiently by linearizing the LLM at the last layer using multinomial logistic regression models. Our approach is computationally efficient, analyzable, and performs well empirically. We demonstrate this on several problems, and back our claims with both quantitative results and an LLM evaluation.

==> section/app_exp.tex <==
We present additional fine-tuning results on two more datasets: (1) Sherlock Holmes dataset and (2) scifi Dataset. As in \cref{sec:experiments} we compare the quality of generated sentences by evaluating using  Claude-3. In Table~\ref{tab:table_app_1} and  \ref{tab:table_app_2} we provide comparison of the our algorithm \tokenod with respect to uniform sampling on Sherlock Holmes and scifi datasets.
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
        Number of Samples ($n$) & 50 & 100 & 200 & 300 & 400 & 500 & 1000 & 2000 & 5000  \\
        \hline
        \begin{tabular}{@{}c@{}} Percentage of times\\Uniform was preferred \end{tabular}  & {41} & 40 &  36 &  37 & 40 & 35 & 43 & 38 & 31\\
        \hline
        \begin{tabular}{@{}c@{}} Percentage of times\\Greedy-OD was preferred \end{tabular} & 59 & 60 & 64 & 63 & 60 & 65 & 57 & 62 & 69 \\
        \hline
    \end{tabular}
    \caption{Comparison between \tokenod  and Uniform Sampling on Sherlock Dataset.}
    \label{tab:table_app_1}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
        Number of Samples ($n$) & 100 & 200 & 300 & 400 & 500 & 1000 & 2000 & 3000 & 5000  \\
        \hline
        \begin{tabular}{@{}c@{}} Percentage of times\\Uniform was preferred \end{tabular}  & {35} & 32 &  26 &  26 & 25 & 34 & 26 & 29 & 35\\
        \hline
        \begin{tabular}{@{}c@{}} Percentage of times\\Greedy-OD was preferred \end{tabular} & 65 & 68 & 74 & 74 & 75 & 66 & 74 & 71 & 65 \\
        \hline
    \end{tabular}
    \caption{Comparison between \tokenod  and Uniform Sampling on scifi Dataset.}
    \label{tab:table_app_2}
\end{table}

==> section/comments.tex <==
\textbf{Objective:} Our objective is to 
each $\x_{i,j} \in \R^d, \forall i, j$, represents a word vector and $T(i)$ is the number of words in sentence $i$. Note that the number of tokens/words in every sentence could potentially be different. Our goal is to to train the model using next word prediction, i.e., given tokens $\x_{i,1}, \x_{i,2},\ldots,\x_{i,t}$, predict the next word $y_{t+1}$. In the context of fine-tuning an LLM, $\x_{i,j}$ represents the features of the pre-logit layer. 

\textbf{Objective}: Our objective is to train the model on a subset of $n$ sentences. One simple approach would be to sample the $n$ sentences uniformly at random from the $N$ sentences. We rather propose a greedy Optimal Design (OD) strategy for sampling sentences with the most information content.

 

{\color{blue}I suggest the following notation:

* We have $N$ sentences. Sentences are indexed by $i \in [N]$. Sentence $i$ has $N_i$ tokens. Tokens in any sentence $i$ are indexed by $j \in [N_i]$.

* We have $L$ distinct tokens. The index of token $j$ in sentence $i$ is $y_{i, j} \in [L]$. Therefore, sentence $i$ is a vector of length $N_i$, $y_i = (y_{i, j})_{j \in [N_i]}$, and the dataset of all $N$ sentences is $\cD = \{y_i\}_{i \in [N]}$.

* A subset of selected sentences is $\cS \subseteq [N]$.

* We also define a representation of history up to token $j$ in sentences $i$, $x_{i, j} \in \mathbb{R}^d$. This is a later to be defined function of $(y_{i, k})_{k \in [j - 1]}$. We define $(y_{i, k})_{k \in [0]} = ()$.

Let
\begin{align}
  \cL_S(\Theta)
  = \sum_{i \in S} \sum_{j = 1}^{N_i} \log p(y_{i, j} \mid x_{i, j}; \Theta)
  \label{loglik}
\end{align}
be the optimized log-likelihood, where $\Theta = (\theta_\ell)_{\ell \in [L]}$. Here $\theta_\ell \in \mathbb{R}^d$ and $\Theta \in \mathbb{R}^{d \times L}$. {\color{red}Define $p(y_{i, j} \mid x_{i, j}; \Theta)$.} \todobin{We need to think of how to include regularization.}

Suppose that the log-likelihood in \eqref{loglik} concentrates at a single point as the number of observations $S$ increases. Then the rate of the concentration can be measured by the curvature of \eqref{loglik} at $\Theta_*$, which can be measured by its Hessian. The Hessian of \eqref{eq:loglik} is
\begin{align}
  \nabla^2 \cL_S(\Theta)
  = \sum_{i \in S} \sum_{j = 1}^{N_i}
  \nabla^2 \log p(y_{i, j} \mid x_{i, j}; \Theta)\,.
  \label{eq:hessian}
\end{align}
{\color{red}Define $\nabla^2 \log p(y_{i, j} \mid x_{i, j}; \Theta)$ and work out the closed from. Double check with Section 10.3 of \url{https://github.com/probml/pml-book/releases/latest/download/book1.pdf}.}

We greedily maximize the log determinant of $\nabla^2 \cL_S(\Theta)$. We would like to stress that the exact maximization is impossible because $\Theta_*$ is unknown. To get around this issue, we bound $\nabla^2 \cL_S(\Theta)$ from below, in the PSD sense, as follows. {\color{red}Derive $\Theta$-independent $c$ in
\begin{align}
  \nabla^2 \log p(y_{i, j} \mid x_{i, j}; \Theta)
  \succeq c \, x_{i, j} x_{i, j}^\top\,.
  \label{eq:lower bound}
\end{align}
Use the assumption that $\|x_{i, j}\|_2 \leq 1$ and $\|\theta_\ell\|_2 \leq 1$.}

The last remaining step is to analyze our approach.


\textbf{Analysis}

We can do a simplified or more complex analysis. I am not sure that we will have time for the latter. Let me start with the bare minimum. The bare minimum is:

1. Extend Section 3 of "Optimal Design for Human Feedback" to covariance matrices $V_\pi = \sum_{i = 1}^N \pi(i) A_i A_i^\top$, where $A_i \in \mathbb{R}^{d \times N_i}$. This should be copy \& paste. Nothing in the proofs uses that $A_i$ have the same number of columns.

2. Extend Lemma 2 and Theorem 3 (Section 4.2) to multinomial logistic regression. You can use any self-normalizing bound to start with. Note that self-normalizing bounds for the bandit setting (adaptive data collection) automatically hold for non-adaptive data collection (our setting). The difference is only in log factors, which we do not care about. The Lipschitz factor of multinomial logistic regression should be $1 / 4$, the same as in logistic regression.

The above gives us guarantees for data logged according to the optimal design. The issue is that we already have a logged dataset and thus maximize $\log\det$ directly. We have two option here:

1. We wing it and informally argue that these are roughly equivalent. This is true.

2. We formally analyze the error. I would proceed as follows:

a. Greedy maximization of $\log\det$ is $1 - 1 / e$ optimal. This allows us to relate the $\log\det$ of our greedy solution and that of the optimal discrete allocation.

b. Assume that the $\log\det$ of the optimal discrete allocation and that of the optimal design (relaxed allocation) are close. In a sense, this says that our dataset has enough diversity. Because of (a), I would go with a multiplicative factor.

c. The above implies that our discrete allocation is similar to that of the optimal design. Therefore, our maximum prediction error decreases at the same rate as that according to the optimal design.

d. Now we chain all claims and get the final bound.}

==> section/greedy.tex <==
\section{Greedy Log-Determinant Maximization}
\label{sec:greedy logdet maximization}

We derive an upper bound on $\normw{\phi_i}{\Sigma_n^{-1}}$, where $\phi_i \in \realset^d$ is a feature vector and $\Sigma_n \in \realset^{d \times d}$ is a design matrix obtained by greedy log-determinant maximization. The result can be summarized as follows. Let $\cD = \set{\phi_i}_{i = 1}^N$ be a dataset of $N$ feature vectors $\phi_i$ such that $\normw{\phi_i}{2} \leq 1$. Let $I_t \in [N]$ be the index of the $t$-th chosen feature vector and $\cS_t = \set{I_\ell}_{\ell = 1}^t$ be the first $t$ chosen feature vectors. Let
\begin{align*}
  \Sigma_t
  = \sigma_0^{-2} I_d + \sum_{i \in \cS_t} \phi_i \phi_i\T\,,
\end{align*}
where $\sigma_0 > 0$ is a constant that guarantees that $\Sigma_0$ is well defined. The $t$-th feature vector is chosen as
\begin{align}
  I_t
  = \argmax_{i \in [N] \setminus \cS_{t - 1}}
  \log\det(\Sigma_{t - 1} + \phi_i \phi_i\T)\,.
  \label{eq:greedy logdet maximization}
\end{align}
{\color{red} Standard error is not sub-modular} Then, under appropriate assumptions,
\begin{align*}
  \max_{i \in [N]} \normw{\phi_i}{\Sigma_n^{-1}}^2
  = \max_{i \in [N]} \phi_i\T \Sigma_n^{-1} \phi_i
  = \tilde{O}(\kappa d / n)\,,
\end{align*}
where $\kappa \geq 1$ characterizes the diversity of dataset $\cD$. We start with the following observation.

\begin{lemma}
\label{lem:variance monotonicity} For any $i \in [N]$ and $t \in [n]$,
\begin{align*}
  \phi_i\T \Sigma_t^{-1} \phi_i
  \leq \phi_i\T \Sigma_{t - 1}^{-1} \phi_i\,.
\end{align*}
\end{lemma}
\begin{proof}
The proof follows from the Sherman–Morrison formula. Specifically, since
\begin{align*}
  \Sigma_t^{-1}
  = \Sigma_{t - 1}^{-1} -
  \frac{\Sigma_{t - 1}^{-1} \phi_i \phi_i\T \Sigma_{t - 1}^{-1}}
  {1 + \phi_i\T \Sigma_{t - 1}^{-1} \phi_i}
  \preceq \Sigma_{t - 1}^{-1}\,,
\end{align*}
we get $v\T \Sigma_t^{-1} v \leq v\T \Sigma_{t - 1}^{-1} v$ for any vector $v \in \realset^d$. This concludes the proof.
\end{proof}

\noindent \cref{lem:variance monotonicity} implies that
\begin{align*}
  \phi_i\T \Sigma_n^{-1} \phi_i
  \leq \frac{1}{n} \sum_{t = 1}^n \phi_i\T \Sigma_{t - 1}^{-1} \phi_i
\end{align*}
holds for any $i \in [N]$. This allows us to attribute the quality of the solution to individual greedy steps in \eqref{eq:greedy logdet maximization}. The next step is to relate $\phi_i\T \Sigma_{t - 1}^{-1} \phi_i$ to $\phi_{I_t}\T \Sigma_{t - 1}^{-1} \phi_{I_t}$. The key observation is that
\begin{align*}
  I_t
  & = \argmax_{i \in [N] \setminus \cS_{t - 1}}
  \log\det(\Sigma_{t - 1} + \phi_i \phi_i\T)
  = \argmax_{i \in [N] \setminus \cS_{t - 1}} \log\det(I_d +
  \Sigma_{t - 1}^{- \frac{1}{2}} \phi_i \phi_i\T \Sigma_{t - 1}^{- \frac{1}{2}}) \\
  & = \argmax_{i \in [N] \setminus \cS_{t - 1}}
  \log(1 + \phi_i\T \Sigma_{t - 1}^{-1} \phi_i)
  = \argmax_{i \in [N] \setminus \cS_{t - 1}}
  \phi_i\T \Sigma_{t - 1}^{-1} \phi_i\,.
\end{align*}
The second equality holds because $\Sigma_{t - 1}$ is fixed when $I_t$ is selected. The last equality holds because the logarithm is a monotone function. It follows that $I_t$ is the index of the feature vector with the maximum variance.

If the scope of the maximization was $i \in [N]$, the inequality $\phi_i\T \Sigma_{t - 1}^{-1} \phi_i \leq \phi_{I_t}\T \Sigma_{t - 1}^{-1} \phi_{I_t}$ would hold for any $i \in [N]$. Since the scope is $i \in [N] \setminus \cS_{t - 1}$, we make the following assumption, which equates to $\cD$ being sufficiently diverse.

\begin{assumption}
\label{ass:diverse feature vectors} There exists a constant $\kappa \geq 1$ such that
\begin{align*}
  \phi_i\T \Sigma_{t - 1}^{-1} \phi_i
  \leq \kappa \phi_{I_t}\T \Sigma_{t - 1}^{-1} \phi_{I_t}
\end{align*}
holds for any $i \in [N]$ and $t \in [n]$.
\end{assumption}

\noindent We also use the following logarithmic transformation.

\begin{lemma}
\label{lem:logarithmic transformation} For any $i \in [N]$ and $t \in [n]$,
\begin{align*}
  \phi_i\T \Sigma_{t - 1}^{-1} \phi_i
  \leq \frac{\sigma_0^2}{\log(1 + \sigma_0^2)}
  \log(1 + \phi_i\T \Sigma_{t - 1}^{-1} \phi_i)\,.
\end{align*}
\end{lemma}
\begin{proof}
We start with an upper bound on $\phi_i\T \Sigma_{t - 1}^{-1} \phi_i$. By Weyl's inequalities, we have
\begin{align*}
  \lambda_1(\Sigma_{t - 1}^{-1})
  = \lambda_d^{-1}(\Sigma_{t - 1})
  \leq \lambda_d^{-1}(\sigma_0^{-2} I_d)
  = \sigma_0^2\,.
\end{align*}
Therefore, under the assumption that $\normw{\phi_i}{2} \leq 1$, we have $\phi_i\T \Sigma_{t - 1}^{-1} \phi_i \leq \sigma_0^2$. Now note that for any $x \in [0, u]$,
\begin{align*}
  x
  = \frac{x}{\log(1 + x)} \log(1 + x)
  \leq \left(\max_{x \in [0, u]} \frac{x}{\log(1 + x)}\right) \log(1 + x)
  = \frac{u}{\log(1 + u)} \log(1 + x)\,.
\end{align*}
Finally, we set $x = \phi_i\T \Sigma_{t - 1}^{-1} \phi_i$ and $u = \sigma_0^2$, and get our claim.
\end{proof}

\noindent Now we apply \cref{ass:diverse feature vectors} and \cref{lem:logarithmic transformation}, use the telescoping property of the sum, and get
\begin{align*}
  \sum_{t = 1}^n \phi_i\T \Sigma_{t - 1}^{-1} \phi_i
  & \leq \kappa \sum_{t = 1}^n \phi_{I_t}\T \Sigma_{t - 1}^{-1} \phi_{I_t}
  \leq \frac{\sigma_0^2 \kappa}{\log(1 + \sigma_0^2)} \sum_{t = 1}^n
  \log(1 + \phi_{I_t}\T \Sigma_{t - 1}^{-1} \phi_{I_t}) \\
  & = \frac{\sigma_0^2 \kappa}{\log(1 + \sigma_0^2)} \sum_{t = 1}^n
  \log\det(I_d + \Sigma_{t - 1}^{- \frac{1}{2}} \phi_{I_t} \phi_{I_t}\T
  \Sigma_{t - 1}^{- \frac{1}{2}}) \\
  & = \frac{\sigma_0^2 \kappa}{\log(1 + \sigma_0^2)} \sum_{t = 1}^n
  \log\det(\Sigma_{t - 1} + \phi_{I_t} \phi_{I_t}\T) - \log\det(\Sigma_{t - 1}) \\
  & = \frac{\sigma_0^2 \kappa}{\log(1 + \sigma_0^2)}
  \sum_{t = 1}^n \log\det(\Sigma_t) - \log\det(\Sigma_{t - 1}) \\
  & = \frac{\sigma_0^2 \kappa}{\log(1 + \sigma_0^2)}
  (\log\det(\Sigma_n) - \log\det(\Sigma_0)) \\
  & = \frac{\sigma_0^2 \kappa}{\log(1 + \sigma_0^2)}
  \log\det(\Sigma_0^{- \frac{1}{2}} \Sigma_n \Sigma_0^{- \frac{1}{2}})\,.
\end{align*}
Furthermore,
\begin{align*}
  \log\det(\Sigma_0^{- \frac{1}{2}} \Sigma_n \Sigma_0^{- \frac{1}{2}})
  & \leq d \log\left(\frac{1}{d}
  \trace(\Sigma_0^{- \frac{1}{2}} \Sigma_n \Sigma_0^{- \frac{1}{2}})\right)
  = d \log\left(1 + \frac{1}{d} \sum_{t = 1}^n
  \trace(\Sigma_0^{- \frac{1}{2}} \phi_{I_t} \phi_{I_t}\T
  \Sigma_0^{- \frac{1}{2}})\right) \\
  & = d \log\left(1 + \frac{1}{d} \sum_{t = 1}^n
  \phi_{I_t}\T \Sigma_0^{-1} \phi_{I_t}\right)
  \leq d \log\left(1 + \frac{\sigma_0^2 n}{d}\right)\,.
\end{align*}
Finally, we combine all claims and get
\begin{align*}
  \max_{i \in [N]} \phi_i\T \Sigma_n^{-1} \phi_i
  \leq \frac{\kappa}{n} \sum_{t = 1}^n \phi_{I_t}\T \Sigma_{t - 1}^{-1} \phi_{I_t}
  \leq \frac{\sigma_0^2 \log\left(1 + \frac{\sigma_0^2 n}{d}\right)}
  {\log(1 + \sigma_0^2)} \frac{\kappa d}{n}\,.
\end{align*}
This concludes the proof.

